Perspectives on Incorporating Expert Feedback into Model Updates

Machine learning (ML) practitioners are increasingly tasked with developing models that are aligned with non-technical experts' values and goals. However, there has been insufficient consideration on how practitioners should translate domain expertise into ML updates. In this paper, we consider how to capture interactions between practitioners and experts systematically. We devise a taxonomy to match expert feedback types with practitioner updates. A practitioner may receive feedback from an expert at the observation- or domain-level, and convert this feedback into updates to the dataset, loss function, or parameter space. We review existing work from ML and human-computer interaction to describe this feedback-update taxonomy, and highlight the insufficient consideration given to incorporating feedback from non-technical experts. We end with a set of open questions that naturally arise from our proposed taxonomy and subsequent survey.

==> Hide/old4and5.tex <==
\section{Stakeholder Feedback} \label{sec:feedback}
Once a stakeholder has observed information about the model, practitioners may ask for feedback to improve the models behavior.  We consider two feedback types: (1) \emph{data}, which collects more points or modifies the datasets; and (2) \emph{property}, which collects desirable properties to append to loss functions.
Additionally, we consider when the feedback style can either be \emph{choices} or \emph{open-ended}; in the former, the stakeholder is explicitly given choices to select from, while the stakeholder can provide any information in the latter.
% In Table \ref{tab:feedback}, we highlight examples of prior work and how they are categorized by feedback style and type.



% \begin{table*}
% \centering
% \begin{tabular}{c|c|c|c|c}
% \toprule
% Paper    & Feedback Prompt & Feedback Style & Feedback Type & Update Type \\ 
% \midrule
% % \citet{berk2018fairness} & \textit{Hola que tal? However, it may be difficult to convert this } & Choice & Data & Data \\
% \citet{lage2018human} & Provide a prediction given the following explanation. & Open-Ended & Property & Constraint \\
% %  & & (Time taken) & (Interpretability) & $\mathcal{L}^{\prime}$ \\
% % \midrule
% \citet{wang2021gam} &  & Open-Ended & Property & Constraint  \\
% \citet{hilgard2021learning} & \textit{TODO} & Property & Property \\
% \citet{jung2019algorithmic} & \textit{Which individual should be treated better?} & Choice & Data & Property\\
% \citet{weinberger2020learning} & \textit{TODO} & unclear& Property & Property\\
% \citet{lee2020limeade} & \textit{Select region of image and indicate if it is a pos/neg predictor} &Open-Ended & Data & Data\\
% % \midrule
% % Equal Accuracy~\citep{berk2018fairness} & \small $f_\text{ea}(\theta) = f_\text{unf}(\theta) = \sum_{j \in \{-1,1\}} |P_{j,a,j} - P_{j,b,j}|$ \\
% % \midrule
% % Equal Opportunity~\citep{hardt2016} & $f_\text{eq}(\theta) =  P_{1,a,1} - P_{1,b,1}$ \\
% % \midrule
% % Equalized Odds~\citep{hardt2016} & $f_\text{eo}(\theta) =  \sum_{j \in \{-1,1\}}  |P_{1,a,j} - P_{1,b,j}|$ \\
% \bottomrule
% \end{tabular}
% \caption{\vccomment{I think we should organize by Feedback+Update Type}}
% \label{tab:feedback}
% \end{table*}


% Such feedback might be qualitative or quantitative. To achieve our goal of improving $\hat \theta$, we distinguish between unusuable feedback and more desirable forms of feedback (which we later connect to preferences that are used to update the model). For each of the above section, illustrate what this is and pros/cons.

% These are usable/concrete/measurable? Overview of query types in the spectrum-- pairwise, property, etc... \vccomment{Make this into a figure: simple example that showcases all four.} The following subsections are presented in the order of our spectrum.


\subsection{Data-driven Feedback}
Upon gaining transparency into $\hat \theta$ and its behavior on specific data points, stakeholder may choose to provide further supervision in the form of new, augmented, or auxiliary data. 
% When soliciting data from stakeholders to improve $\hat \theta$, practitioners may elect to use a visualization, as in Figure..., or prompt the stakeholder to provide data of a specific sort. /vccomment{this belongs in section 3.2}

A stakeholder might elect to add new labeled data to the training set~\cite{fanton2021human}.
The active learning community has long studied the problem how to identify regions of input space where additional training data is required and how to best label such data. Stakeholders have been asked to provide labels for data in regions with high epistemic uncertainty~\cite{wan2020human}, low representation~\cite{fu2013survey}, etc. In much of this work, practitioners generate synthesize new data using generative modelling techniques and ask stakeholders to review the generated points. Stakeholders have also been asked to relabel misclassifications~\cite{kaushik2019learning} and down-weight ``unhelpful'' data points~\cite{ryazanov2021deep}. 
In semi-supervised learning, stakeholders might provide additional unlabeled data which is then pseudo-labeled~\cite{carmon2019unlabeled,arazo2020pseudo}.

\ubcomment{any missing forms of \textbf{feedback} not update?}


\noindent\textbf{Pros. } The most natural thing to do is often to collect additional data to be ensure the model is more representative of the task being automated.% \vccomment{elaborate?}


\noindent\textbf{Cons. } Since data-driven feedback is a more granular piece of feedback that can be provided, it might be the case that a lot of data will need to be collected in order to make a more drastic change to the model further in the pipeline.

\subsection{Property-driven Feedback}

Another way that a stakeholder may provide feedback is through specification of property-level feedback. This type of feedback can be broadly considered as higher level feedback on the behavior of the model, rather than feedback on the model's behavior at specific instances. 
One example of a property-driven feedback is explicit feedback over a set of good models. \citet{lage2018human} observes how quickly stakeholders can predict the model's output from an explanation: the quicker the response, the better the explanation.

Another way to solicit property-driven feedback is at the constraint level. There are a number of prior work that study how to optimize for constraints, but in general it is not clear how to ask users for open-ended feedback at the constraint level. One example of a constraint that could be prompted from stakeholders is how to preprocess the data in a way that would align with the stakeholder goal. For example, in the fairness literature data pre-processing can be used to reduce discrimination \citep{hajian2012methodology,feldman2015certifying, calmon2017optimized}. We discuss how pre-processing would be used as a model update in Section~\ref{sec:updates}.

Finally, a common way that property-driven feedback can manifest is through side information for a task. Here, every datapoint $(x_i, y_i)$ is accompanied by an auxiliary piece of information $s_i$ that can be used during learning.
Side information might include feature attributions~\cite{weinberger2020learning}, style factors~\cite{adel2018discovering}, semantically meaningful concepts~\cite{koh2020concept}, privileged information~\cite{vapnik2015learning}, or explanations~\cite{hind2019ted}. While many works have used side information at train time, few have discussed how to solicit side information from stakeholders.
\ubcomment{add examples}

% \vccomment{attribution prior \citep{weinberger2020learning}, CBM \citep{koh2020concept}}.


Additionally, property-level feedback may be challenging for stakeholders to specify. For example, stakeholders may have desired properties corresponding to societal norms / ethics (e.g., \vccomment{todo}). However, it may be difficult to convert this into a precise statement that can be used to update $\mathcal{D}$ or $\mathcal{L}$. 


\noindent\textbf{Pros. } Property-level changes are more high-level and could lead to a larger change in the model. \vccomment{elaborate?}

\noindent\textbf{Cons. } As evidenced by the lack of prior work that actually ask for property-level feedback, this type of feedback may be more difficult to solicit from stakeholders because it is difficult to accurately provide the transparency step (i.e., having a presentation that accurately captures the intended content). For example, it might be challenging to present two model choices to a stakeholder rather than two error choices. The latter is much easier to visualize.




% \begin{itemize}
%     \item Might be difficult for the human to specify. Societal norms? What the human wants is not necessarily and immediately quantifiable/optimizable (this is important, and an open question). 
%     \item B
% \end{itemize}



% \subsection{Choice-driven Feedback}

% Choice-driven feedback is feedback presented to the stakeholder in the form of options. In general, the stakeholder picks one of the presented options. However, it may also be possible for the stakeholder to pick multiple options or rank the options. Both data-driven and property-driven feedback can also be presented as choices. An example of a data-level choice is the choice between errors. For example \vccomment{talk about fairness paper here.} An example of a property-level choice is \vccomment{talk about rashomon sets}.

% %Rashomon set over error or properties or model


% \noindent\textbf{Pros. } In existing work, pairwise feedback particularly at the data level (in the form of choices over errors) is common \vccomment{cite examples}. This is because it might be easier in many cases for humans to \emph{choose} between options than come up with a correct answer themselves.

% \noindent\textbf{Cons. } At the property-level, it may be difficult for the stakeholder to pick between options largely because it is difficult to accurately provide the transparency step (i.e., having a presentation that accurately captures the intended content). For example, it might be more challenging to present two model choices to a stakeholder rather than two error choices. The latter is much easier to visualize.

% Additionally, when aggregating a set of choices, it may be the case that the choices are \emph{inconsistent}. \vccomment{clarify what this means and cite social choice lit.}



\section{Model Updates} \label{sec:updates}

Once stakeholders have provided their feedback, we discuss how practitioners can leverage stakeholder input to improve the $\hat \theta$. We first overview the two main types of updates (observation and constraint). Note that while we provide a number of examples of both types of update, we emphasize that for the most part the relevant work that we cite \emph{do not} involve contain the feedback portion (i.e., have a stakeholder in the loop). Thus, we then provide an extensive discussion that illustrates how the two types of feedback provided by the stakeholders can be converted into the two common update types. A primary challenge we foresee for HILL is how to effectively transform the stakeholder's feedback into usable model updates.

\subsection{Update by observation }
\vccomment{Remainder of write-up is under construction.}
One sensible way to incorporate feedback into the model is by changing the dataset from $\mathcal{D}$ to $\mathcal{D}^{\prime}$. 
\begin{equation}
    \tilde{\theta} = \argmin_{\theta \in \Theta} \sum_{(x,y) \in \mathcal{D}^{\prime}} \mathcal{L}(x,y;\theta).
\end{equation}

Examples might include: weak supervision, data augmentation, machine unlearning / influence function, relabeling /label smoothing / label denoising, generating data.

% \vccomment{in general adding data is trivial}
% \vccomment{compare when people reweight vs add more data}
% \vccomment{should we discuss generating more data here?}

\citep{plumb2021finding, lee2020explanation, weinberger2020learning}


\subsection{Update by constraint } 
Another way to incorporate feedback into the model is by adding a constraint to the optimization objective. This manifests as a change in the loss function from $\mathcal{L}$ to $\mathcal{L}^{\prime}$. 
%Constraint updates manifest in the form of a change to the loss function. 

\begin{equation}
    \tilde{\theta} = \argmin_{\theta \in \Theta} \sum_{(x,y) \in \mathcal{D}} \mathcal{L}^{\prime}(x,y;\theta).
\end{equation}


\begin{enumerate}
\item \citep{zafar2017fairness, lage2018human}
\item \href{https://ojs.aaai.org/index.php/AAAI/article/view/9014
}{Active Learning with Model Selection}
\item \href{Learning Soft Constraints from Demonstrations for IRL}{https://arxiv.org/abs/2109.11018}
\item representations: madry editing, \citep{hilgard2021learning}
\end{enumerate}

\begin{itemize}
    \item \textbf{Interpretability} (regularizing feature attributions): $\mathcal{R_{\text{int}}} \coloneqq \sum_{x_i \in \mathcal{D}} \sum_{j \in d} g(\theta;x_i)_j - a_{ij}$ where $A \in \mathcal{R}^{n\times d}$ is the desired attribution and $g$ is the explanation function
    \item \textbf{Fairness} (regularizing for disparity): $\mathcal{R_{\text{fair}}} \coloneqq \sum_{\text{pos}} \mathcal{L}(\theta, x_i) - \sum_{\text{neg}} \mathcal{L}(\theta, x_i)$, where $A \in \{\text{pos}, \text{neg}\}$ is the sensitive attribute
    \item \textbf{Domain shift} (regularizing for performance on additional data): $\mathcal{R_{\text{domain}}} \coloneqq \sum_{x_i \in A} \mathcal{L}(\theta, x_i)$, where $A \in \mathcal{R}^{n\times d}$ is additional data \ubcomment{Does this belong in 5.1 or 5.2? This definition implies that we are simply changing $\mathcal{D}$}
\end{itemize}


\textbf{Other Types Updates}
These are less common: change learning algorithm / hypothesis class / parameters. In general it might be more difficult for a stakeholder to provide such technical feedback.


\subsection{Converting Feedback to Update}

A major role of the practitioner in the HILL pipeline is to bridge the gap between the provided stakeholder feedback and the model update, which as evidenced in the prior sections can greatly differ in presentation and form. In general, if a data-driven feedback is provided, it is fairly straightforward to update $\mathcal{D}$ (similarly for property-driven feedback to be used as constraints). However, we find that it is possible to also convert one type of feedback into a model update of the other kind.  While there is not a uniform way to do so, we overview some examples:

\textbf{Data-to-Property: } \citet{jung2019algorithmic} ask stakeholders questions at the individual data level to choose one of the following options when evaluating between two individuals A and B: \textit{no constraint}, \textit{A should be treated as well as B or better}, \textit{B should be treated as well as A or better}, \textit{A and B should be treated equally}. The feedback from the stakeholders to these questions is used to generate a constraint for ERM. \vccomment{elaborate on what the constraint is.}

\citet{hilgard2021learning} constructs a dataset of human decisions based on an interactive representation of the model (model transparency). \vccomment{elaborate on this.}

\vccomment{Hoda paper.}

\textbf{Property-to-Data: } \citet{plumb2021finding} ask stakeholders to identify spurious patterns, which we consider to be a property level feedback. The identified patterns are then used to generate counterfactuals at the data level to incorporate for retraining.  

\vccomment{I think data preprocessing should be another property-to-data.}

